AutoDSE: Enabling Software Programmers to Design Efficient FPGA Accelerators

Adopting FPGA as an accelerator in datacenters is becoming mainstream for customized computing, but the fact that FPGAs are hard to program creates a steep learning curve for software programmers. Even with the help of high-level synthesis (HLS), accelerator designers still have to manually perform code reconstruction and cumbersome parameter tuning to achieve the optimal performance. While many learning models have been leveraged by existing work to automate the design of efficient accelerators, the unpredictability of modern HLS tools becomes a major obstacle for them to maintain high accuracy. To address this problem, we propose an automated DSE framework-AutoDSE- that leverages a bottleneck-guided coordinate optimizer to systematically find a better design point. AutoDSE detects the bottleneck of the design in each step and focuses on high-impact parameters to overcome it. The experimental results show that AutoDSE is able to identify the design point that achieves, on the geometric mean, 19.9x speedup over one CPU core for Machsuite and Rodinia benchmarks. Compared to the manually optimized HLS vision kernels in Xilinx Vitis libraries, AutoDSE can reduce their optimization pragmas by 26.38x while achieving similar performance. With less than one optimization pragma per design on average, we are making progress towards democratizing customizable computing by enabling software programmers to design efficient FPGA accelerators.

==> code/code-cnn-hls.tex <==
\begin{lstlisting}[language=C,caption=CNN HLS C Code Snippet\label{code:cnn_hls},
    float,floatplacement=H]
// Skip const variable initizalization due to page limit
#define input(j, h, w) \
    input[((j) * InImSize * InImSize + (h) * InImSize + (w))]
// Skip the rest due to page limit
 
void CnnKernel(
     const float* input $\circled{\small 1}$, const float weight$\circled{\small 1}$, 
     const float* bias $\circled{\small 1}$, float* output $\circled{\small 1}$) {
#pragma HLS INTERFACE m_axi port=input bundle=gmem1 
#pragma HLS INTERFACE s_axilite port=input bundle=control
// Skip other interface pragmas due to page limit

  float C[ImSize][ImSize];
  for (int i = 0; i < NumOut; ++i) { $\circled{\small 4}$ $\circled{\small 6}$
    // Initialization
    for (int h = 0; h < ImSize; ++h) {
      for (int w = 0; w < ImSize; ++w)
        C[h][w] = bias[i];
    }
    // Convolution
    for (int j = 0; j < NumIn; ++j) { $\circled{\small 5}$
      for (int h = 0; h < ImSize; ++h) { $\circled{\small 5}$
        for (int w = 0; w < ImSize; ++w) { $\circled{\small 5}$
          for (int p = 0; p < kKernel; ++p) { $\circled{\small 5}$
            for (int q = 0; q < kKernel; ++q) $\circled{\small 5}$
              C[h][w] += weight(i, j, p, q) * input(j,h + p,w + q); $\circled{\small 2}$ $\circled{\small 3}$ $\circled{\small 6}$
     } } } }
    // ReLU
    for (int h = 0; h < ImSize; ++h) { $\circled{\small 5}$
      for (int w = 0; w < ImSize; ++w) { $\circled{\small 5}$
        C[h][w] = max(0.f, C[h][w]);
    } }
    // Max pooling
    for (int h = 0; h < OutImSize; ++h) { $\circled{\small 5}$
      for (int w = 0; w < OutImSize; ++w) { $\circled{\small 5}$
        output(i,h,w) = max(
            max(C[h * 2][w * 2    ], C[h * 2 + 1][w * 2    ]),
            max(C[h * 2][w * 2 + 1], C[h * 2 + 1][w * 2 + 1]));
} } } }

\end{lstlisting}

==> code/code-cnn.tex <==
\begin{lstlisting}[language=C,caption=Part of HLS C Code Snippet for Convolution Layer\label{code:cnn},float,floatplacement=H]
    // Skip due to page limit. 
for (int i = 0; i < NumOut; i++){
  ...
  for (int j = 0; j < NumIn; ++j) {
    for (int h = 0; h < ImSize; ++h) {
      for (int w = 0; w < ImSize; ++w) {
        for (int po = 0; po < ParallelOut; po++){
          float tmp = 0;
          for (int p = 0; p < kKernel; ++p) {
            for (int q = 0; q < kKernel; ++q) {
              tmp += weight[(i << shift) + po][j][p][q] * input[j][h + p][w + q];
            } }
          out[po][h][w] += tmp;
} } } } }
    // Skip due to page limit. 
\end{lstlisting}







==> code/code-hls-opt.tex <==
\begin{lstlisting}[
    caption=N-W HLS C Code Snippet with Manual Optimization\label{code:hls_opt},
    float,floatplacement=b]
void NW(...) {
  int M[129][129];
#pragma HLS array_partition variable=M cyclic factor=4 dim=1  
  ...
  for(i=0; i<129; i++) { $\circled{\small 5}$
#pragma HLS pipeline
#pragma HLS unroll factor=8
    M[0][i] = ..,;     
  }
  for(j=0; j<129; j++) { $\circled{\small 5}$
#pragma HLS pipeline  
#pragma HLS unroll factor=8
    M[j][0] = ...; 
  }
  for(i=1; i<129; i++) {
    for(j=1; j<129; j++) { $\circled{\small 5}$
#pragma HLS pipeline
#pragma HLS unroll factor=8
      M[i][j] = ...
  }}
  ...
}
void compute(char seqAs[32][16][8], char seqBs[32][16][8],
               char alignedAs[32][8][32] char alignedBs[32][8][32]) {
#pragma HLS inline off
  for (int i=0; i<32; i++) { $\circled{\small 4}$
#pragma HLS unroll
    NW(seqAs[i], seqBs[i], alignedAs[i], alignedBs[i]);
}}
void load(...) { ... } // off-chip data load
void store(...) { ... } // off-chip data store
void kernel(int batch, ap_uint<512> $\circled{\small 1}$ seqAs[], ap_uint<512> $\circled{\small 1}$ seqBs[],
            ap_uint<512> $\circled{\small 1}$ alignedAs[], ap_uint<512> $\circled{\small 1}$ alignedBs[]) {
#pragma HLS INTERFACE m_axi port=seqAs offset=slave
#pragma HLS INTERFACE m_axi port=seqBs offset=slave
#pragma HLS INTERFACE m_axi port=alignedAs offset=slave
#pragma HLS INTERFACE m_axi port=alignedBs offset=slave
#pragma HLS INTERFACE s_axilite port=seqAs offset=control
#pragma HLS INTERFACE s_axilite port=seqBs offset=control
#pragma HLS INTERFACE s_axilite port=alignedAs offset=control
#pragma HLS INTERFACE s_axilite port=alignedBs offset=control

  char seqAs_buf_0[32][16][8]; $\circled{\small 3}$
#pragma HLS array_partition var=seqAs_buf_0 complete dim=1
#pragma HLS array_partition var=seqAs_buf_0 complete dim=3
  // the declarations for the other buffers are omitted
  for (int i=0; i<batch/32+2; i++) {
    if (i \% 2 == 0) { 
      load(/* seqAs_buf_0 <= seqAs, seqBs_buf_0 <= seqBs */); $\circled{\small 2}$ 
      compute(seqAs_buf_1, seqBs_buf_1, alignedAs_buf_1, alignedBs_buf_1)
      store(/* alignedAs_buf_0 <= alignedAs, alignedBs_buf_0 <= alignedBs */); $\circled{\small 2}$ $\circled{\small 3}$
    }
    else { 
      load(/* seqAs_buf_1 <= seqAs, seqBs_buf_1 <= seqBs */); $\circled{\small 2}$
      compute(seqAs_buf_0, seqBs_buf_0, alignedAs_buf_0, alignedBs_buf_0)
      store(/* alignedAs_buf_1 <= alignedAs, alignedBs_buf_1 <= alignedBs */); $\circled{\small 2}$ $\circled{\small 3}$
}}}
\end{lstlisting}

==> code/code-vitis.tex <==
\begin{lstlisting}[caption=The code snippet form \texttt{remap} kernel in Vitis Library\label{code:vitis},
    float,floatplacement=H]
// Skip due to page limit
ap_uint<64> bufUram[PLANES][WIN_ROW][(COLS + 7) / 8];
#pragma HLS ARRAY_PARTITION variable=bufUram complete dim=2
#pragma HLS ARRAY_PARTITION variable=bufUram complete dim=1
XF_TNAME(SRC_T, NPC) sx8[8];
#pragma HLS ARRAY_PARTITION variable=sx8 complete dim=1

loop_height:
    for (int i = 0; i < rows + ishift; i++) {
#pragma HLS LOOP_FLATTEN OFF
#pragma HLS LOOP_TRIPCOUNT min=1 max=row_tripcount

    loop_width:
        for (int j = 0; j < cols; j++) {
#pragma HLS PIPELINE II=1
#pragma HLS dependence variable=buf     inter false
#pragma HLS dependence variable=bufUram inter false
#pragma HLS dependence variable=r       inter false
#pragma HLS LOOP_TRIPCOUNT min=1 max=COLS

            if (i < rows && j < cols) {
                s = src.read(read_pointer_src++);
                if (USE_URAM) {
                    sx8[j % 8] = s;
                    for (int pl = 0, bit = 0; pl < PLANES; pl++, bit += 8) {
#pragma HLS UNROLL
                        for (int k = 0; k < 8; k++) {
#pragma HLS UNROLL
                            bufUram[pl][i % WIN_ROW][j / 8](k * 8 + 7, k * 8) = sx8[k](bit + 7, bit);
            }   }   }   }

            if (!USE_URAM) buf[i % WIN_ROW][j] = s;
            r[i % WIN_ROW] = i;
            if (i >= ishift) {
                float mx_fl = mapx.read_float(read_pointer_map);
                float my_fl = mapy.read_float(read_pointer_map++);

                int x = (int)(mx_fl + 0.5f);
                int y = (int)(my_fl + 0.5f);

                bool in_range = (y >= 0 && my_fl <= (rows - 1) && r[y % WIN_ROW] == y && x >= 0 && mx_fl <= (cols - 1));
                if (in_range)
                    if (USE_URAM) {
                        XF_TNAME(DST_T, NPC) dx9[8];
#pragma HLS ARRAY_PARTITION variable=dx9 complete dim=1
                        for (int pl = 0, bit = 0; pl < PLANES; pl++, bit += 8) {
                            ap_uint<72> tempvalue[PLANES]; //
                            tempvalue[pl] = bufUram[pl][y % WIN_ROW][x / 8];
                            for (int k = 0; k < 8; k++) {
                                dx9[k](bit + 7, bit) = tempvalue[pl].range(k * 8 + 7, k * 8);
                        }   }
                        d = dx9[x % 8];
                    } else
                        d = buf[y % WIN_ROW][x];
                else
                    d = 0;
                dst.write(write_pointer++, d);
    }   }   }
// Skip due to page limit
\end{lstlisting}






==> figures/fig-ds-building.tex <==
\begin{figure}[!tbh]
	\centering
	\includegraphics[width=\linewidth]{./figures/ds_building_cache.pdf} 
	\caption{Graph-based Design Space Building Approach}
	\label{fig:ds_building}
\end{figure}

==> figures/fig-exp-hybrid.tex <==
\begin{figure*}[!htb]
	\centering
	\includegraphics[width=\linewidth]{./figures/exp_all.pdf} 
	\caption{Speedup of the Proposed Approach, S2FA~\cite{s2fa}, Out-of-Box and Manual Design Over an Intel Xeon CPU Core}
	\label{fig:exp_hybrid}
\end{figure*}

==> figures/fig-exp-summary.tex <==
\begin{figure}[!tbh]
	\centering
	\includegraphics[width=\linewidth]{./figures/exp_summary.pdf} 
	\caption{Summary of Overall Speedup and DSE Time}
	\label{fig:exp_summary}
\end{figure}
